The formation of peptide-like molecules on interstellar dust grains

Molecules with an amide functional group resemble peptide bonds, the molecular bridges that connect amino acids, and may thus be relevant in processes that lead to the formation of life. In this study, the solid state formation of some of the smallest amides is investigated in the laboratory. To this end, CH$_{4}$:HNCO ice mixtures at 20 K are irradiated with far-UV photons, where the radiation is used as a tool to produce the radicals required for the formation of the amides. Products are identified and investigated with infrared spectroscopy and temperature programmed desorption mass spectrometry. The laboratory data show that NH$_{2}$CHO, CH$_{3}$NCO, NH$_{2}$C(O)NH$_{2}$, CH$_{3}$C(O)NH$_{2}$ and CH$_{3}$NH$_{2}$ can simultaneously be formed. The NH$_{2}$CO radical is found to be key in the formation of larger amides. In parallel, ALMA observations towards the low-mass protostar IRAS 16293-2422B are analysed in search of CH$_{3}$NHCHO (N-methylformamide) and CH$_{3}$C(O)NH$_{2}$ (acetamide). CH$_{3}$C(O)NH$_{2}$ is tentatively detected towards IRAS 16293-2422B at an abundance comparable with those found towards high-mass sources. The combined laboratory and observational data indicates that NH$_{2}$CHO and CH$_{3}$C(O)NH$_{2}$ are chemically linked and form in the ice mantles of interstellar dust grains. A solid-state reaction network for the formation of these amides is proposed.

==> general.tex <==
%
% Editing
%
\newcommand\cits[1]{Sec.~\ref{sec:#1}}
\newcommand\labs[1]{\label{sec:#1}}

\def \red#1{\textcolor{red}{#1}}
\def \blue#1{\textcolor{blue}{#1}}
\def \vert#1{\textcolor{green}{#1}}
\def \jaune{\textcolor{yellow}}
\def \magenta#1{\textcolor{magenta}{#1}}
\def \cyn#1{\textcolor{cyan}{#1}}
\def \etc{{\it etc}}
\def \ie{{\it i.e.}}
\def \eg{{\it e.g.}}
\def \via{{\it via}}
\def \idem{{\it idem}}
\def \infine{{\it in fine}}
\def \apost{{\it a posteriori}}
\def \afort{{\it a fortiori}}
\def \vs{{\it vs}}
\def \etal{{\it et al}}
\def \cad{c'est-\`a-dire}
\newcommand{\permil}{%
  \relax\ifmmode\promillezeichen
        \else\leavevmode\(\mathsurround=0pt\promillezeichen\)\fi}
\newcommand{\perth}{\textperthousand}
\newcommand\mydate{}
\edef\mydate{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
%
%-----------------------------------------------
% Mathematics
%\DeclareMathOperator{\sinc}{sinc}
\newcommand\sinc{{\rm sinc}}
\def \dix#1{\ensuremath{{\,\rm 10^{#1}}}}
\def \tdix#1{\ensuremath{{\,\times 10^{#1}}}}
\def \dth{\ensuremath{\ud\theta}}
\def \dph{\ensuremath{\ud\phi}}
\def \om{\ensuremath{{\Omega}}}
\def \dom{\ensuremath{\ud\om}}
\def \ohalf{\ensuremath{\Omega_{2\pi}}}
\def \ud   {\ensuremath{\,\mathrm{d}}}
\def \uD   {\ensuremath{\,\mathrm{D}}}
\def \udp  {\ensuremath{\partial}}
\def \dt#1{\ensuremath{\frac{d{#1}}{dt}}}
\def \dtot#1#2{\ensuremath{\frac{d{#1}}{d{#2}}}}
\def \dpdt#1{\ensuremath{\frac{\partial{#1}}{\partial{t}}}}
\newcommand\dpartij[3]{\ensuremath{\partial^{#2}_{#1}#3}}
\newcommand\dpart[2]{\ensuremath{\partial_{#1}#2}}
\def \nbb{\ensuremath{{\rm I\!N}}} % ensemble des entiers
\def \rbb{\ensuremath{{\rm I\!R}}} % ensemble des reels
\def \dint {\displaystyle\int}
\def \dsum {\displaystyle\sum}
\newcommand \fracp[2]{\ensuremath{\left(\frac{#1}{#2}\right)}}
\newcommand \fracc[2]{\ensuremath{\left[\frac{#1}{#2}\right]}}
\def \lp   {\ensuremath{\left(}}
\def \rp   {\ensuremath{\right)}}
\def \lc   {\ensuremath{\left[}}
\def \rc   {\ensuremath{\right]}}
\def \lb   {\ensuremath{\left\{}}
\def \rb   {\ensuremath{\right\}}}
\def \aver#1{\ensuremath{\langle #1 \rangle}}
\def \<{\ensuremath{\langle}}
\def \>{\ensuremath{\rangle}}
\def \lr{\ensuremath{\leftrightarrow}}
\def \lra{\ensuremath{\longrightarrow}}
\def \ra{\ensuremath{\rightarrow}}
\def \la{\ensuremath{\leftarrow}}
\def \Ra{\ensuremath{\Rightarrow}}
\def \LRa{\ensuremath{\Leftrightarrow}}
\def \vdot#1#2{\ensuremath{\vect{{#1}}\cdot\vect{{#2}}}}
\def \vcro#1#2{\ensuremath{\vect{{#1}}\times\vect{{#2}}}}
\def \rot{\ensuremath{\vect{\nabla}\times}}
\def \div#1{\ensuremath{\vect{\nabla}\cdot{#1}}}
\def \grad#1{\ensuremath{\vect{\nabla}(#1)}}
\def \lapla{\ensuremath{\nabla^2}}
\def \scal#1#2{\ensuremath{\vec{#1}\cdot\vec{#2}}}
\newcommand\logd{\ensuremath{\log_{10}}}
\newcommand\cplx[1]{\ensuremath{\underline{#1}}}
\newcommand\ccplx[1]{\ensuremath{\cplx{#1}^*}}
%
%
%
% ------------------------------------------------------------
%
% Physics and chemistry
%
\def \kb{\ensuremath{k_B}} % {\rm B}}}
\def \vth{\ensuremath{{v_{\rm th}}}}
\newcommand\bpos{\ensuremath{B_\perp}}
\newcommand\blos{\ensuremath{B_\parallel}}
%
%
% ------------------------------------------------------------
%
% General units
%
\def \hz{\ensuremath{{\rm Hz^{-1}}}}
\def \ang{\ensuremath{{\rm \mathring{A}}}}
\def \micr{\ensuremath{\mu {\rm m}}}
\def \pc{\ensuremath{{\rm pc}}}
\def \au{\ensuremath{{\rm AU}}}
\def \ua{\ensuremath{{\rm UA}}}
\def \K{\ensuremath{{\rm K}}}
\def \per#1{\ensuremath{\,{\rm #1}^{-1}}}
\def \unit#1#2{\ensuremath{\,{\rm #1}^{#2}}}
\def \muG{\ensuremath{\mu {\rm G}}}
\def \mmm{\ensuremath{{\,\rm m^{-3}}}}
\def \mm{\ensuremath{{\,\rm m^{-2}}}}
\def \perm{\ensuremath{{\,\rm m^{-1}}}}
\def \percm{\ensuremath{{\,\rm cm^{-1}}}}
\def \cc{\ensuremath{{\,\rm cm^{-2}}}}
\def \ccc{\ensuremath{{\,\rm cm^{-3}}}}
\def \cccs{\ensuremath{\,\rm cm^3\,s^{-1}}}
\def \gccc{\ensuremath{{\,\rm g\,cm^{-3}}}}
\def \cm{\ensuremath{{\,\rm cm}}}
\def \cmm{\ensuremath{{\,\rm cm^2}}}
\def \cmmm{\ensuremath{{\,\rm cm^3}}}
\def \ctwo{\ensuremath{{\,\rm cm^2}}}
\def \cthr{\ensuremath{{\,\rm cm^3}}}
\def \mtwo{\ensuremath{{\,\rm m^2}}}
\def \mthr{\ensuremath{{\,\rm m^3}}}
\def \pers{\ensuremath{{\,\rm s^{-1}}}}
\def \perm{\ensuremath{{\,\rm min^{-1}}}}
\def \perh{\ensuremath{{\,\rm hr^{-1}}}}
\def \peryr{\ensuremath{{\,\rm yr^{-1}}}}
\def \peran{\ensuremath{{\,\rm an^{-1}}}}
\def \yr{\ensuremath{{\,\rm yr}}}
\def \an{\ensuremath{{\,\rm an}}}
\def \cms{\ensuremath{{\,\rm cm\,s^{-1}}}}
\def \ms{\ensuremath{{\,\rm m\,s^{-1}}}}
\def \cmss{\ensuremath{{\,\rm cm\,s^{-2}}}}
\def \mss{\ensuremath{{\,\rm m\,s^{-2}}}}
\def \kms{\ensuremath{{\rm\,km\,s^{-1}}}}
\def \mstar{\ensuremath{M_\star}}
\def \rstar{\ensuremath{R_\star}}
\def \lstar{\ensuremath{L_\star}}
\def \rsol{\ensuremath{R_{\odot}}}
\def \lsol{\ensuremath{L_{\odot}}}
\def \msol{\ensuremath{{M_{\odot}}}}
\def \msolpc{\ensuremath{M_{\odot}\,{\rm pc}^{-1}}}
\def \cckms{\ensuremath{{\rm\,cm^{-2}\,(km/s)^{-1}}}}
\def \kmspc{\ensuremath{{\rm\,km\, s^{-1}\,pc^{-1}}}}
\def \cccK{\ensuremath{{\rm\,cm^{-3}\,\K^{-1}}}}
\def \kkms{\ensuremath{{\rm\,K\,km\,s^{-1}}}}
\def \cmcmg{\ensuremath{{\rm\,cm^2\,g^{-1}}}}
\newcommand{\ccg}{\ensuremath{\rm\,cm^2\,g^{-1}}}
\newcommand{\gcc}{\ensuremath{\rm\,g\,cm^{-2}}}
\def \mmkg{\ensuremath{{\rm\,m^2\,kg^{-1}}}}
\def \mkkms{\ensuremath{\rm\,mK\kms}}
\def \ster{\ensuremath{{\rm\,sr}^{-1}}}
%
% Astrophysics
\def \gam{\ensuremath{\gamma}-ray}
\def \vlsr{\ensuremath{v_{{\rm LSR}}}}
\def \arcmin{\ensuremath{^{\scriptscriptstyle\prime}}}
\def \arcsec{\ensuremath{^{\scriptscriptstyle\prime\prime}}}
\def \degr{\ensuremath{{^{\circ}}}}
\def \hms#1#2#3{\ensuremath{{\,\rm {#1}^h{#2}^m{#3}^s}}}
\def \dms#1#2#3{\ensuremath{{#1}^{\circ}{#2}\arcmin{#3}\arcsec}}
\def \lii{\ensuremath{\ell_{{\rm II}}}}
\def \bii{\ensuremath{b_{{\rm II}}}}
\def \Nh{\ensuremath{N_{{\rm H}}}}
\def \Nhi{\ensuremath{N_{{\rm HI}}}}
\def \Nhh{\ensuremath{N_{{\rm H_2}}}}
\def \av{\ensuremath{A_{{\rm V}}}}
\def \ak{\ensuremath{A_{{\rm K}}}}
\def \ebv{\ensuremath{E_{{\rm B-V}}}}
\def \nh{\ensuremath{n_{{\rm H}}}}
\def \nhh{\ensuremath{n_{{\ce{H2}}}}}
\def \mh{\ensuremath{m_{{\rm H}}}}
%
% Astrochemistry
%
\def \reac#1#2{\begin{equation}\label{eq:#1}\ce{#2}\end{equation}}
\def \reacnn#1{\[\ce{#1}\]}
\def \form#1{\ensuremath{\Phi(\ce{#1})}}
\def \dest#1{\ensuremath{\Delta(\ce{#1})}}
\def \tw   {\ensuremath{^{12}}}
\def \th   {\ensuremath{^{13}}}
\def \twc  {\ce{^{12}C}}
\def \thc  {\ce{^{13}C}}
\def \hep  {\ensuremath{{\rm He^+}}}
\def \hii  {\ensuremath{{\rm \textsc{HII}}}}
\def \hi   {\ensuremath{{\rm \textsc{HI}}}}
\def \hh   {\ensuremath{{\ce{H2}}}}
\def \h    {\ensuremath{{\rm H}}}
\def \hp   {\ensuremath{{\rm H^+}}}
\def \hhp  {\ensuremath{{\rm H_2^+}}}
\def \hhhp {\ensuremath{{\rm H_3^+}}}
\def \hho  {\ensuremath{{\rm H_2O}}}
\def \hcop {\ensuremath{{\rm HCO^+}}}
\def \hthcop {\ensuremath{{\rm H\thc O^+}}}
\def \co   {\ensuremath{{\rm CO}}}
\def \sixo   {\ensuremath{{\rm ^{16}O}}}
\def \eigo   {\ensuremath{{\rm ^{18}O}}}
\def \twCO {\ensuremath{{\rm ^{12}CO}}}
\def \thCO {\ensuremath{{\rm ^{13}CO}}}
\def \cdo  {\ensuremath {{\rm C^{18}O}}}
\def \cdso {\ensuremath {{\rm C^{17}O}}}
\def \thcdo{\ensuremath {{\rm ^{13}C^{18}O}}}
\def \thcp {\ensuremath {{\rm ^{13}C^+}}}
\def \cp   {\ensuremath {{\rm ^{12}C^+}}}
\def \chp  {\ensuremath {{\rm CH^+}}}
\def \cch  {\ensuremath {{\rm C_2H}}}
\def \cfp  {\ensuremath {{\rm CF^+}}}
\def \hf   {\ensuremath {{\rm HF}}}
\def \chhp {\ensuremath {{\rm CH_2^+}}}
\def \chhhp{\ensuremath {{\rm CH_3^+}}}
\def \htco {\ensuremath {{\rm H^{13}CO^{+} }}}
\def \dcop {\ensuremath {{\rm DCO^{+} }}}
% N bearing species
\def \nhhh {\ensuremath {{\rm NH_3}}}
\def \nnhp {\ensuremath {{\rm N_2H^{+}}}}
\def \nht  {\ensuremath {{\rm NH}_3}}
\def \nn   {\ensuremath {{\rm N_2 }}}
\def \cn   {\ensuremath {{\rm CN}}}
%\def \thcn {\ensuremath {{\rm ^{13}CN}}}
\def \thcn {\ce{^{13}CN}}
\def \foun {\ce{^{14}N}}
\def \fifn {\ce{^{15}N}}
\def \dens#1{\ensuremath{n(\ce{#1})}}
\def \ab#1{\ensuremath{[\ce{#1}]}}
%
%
% Fourier transform
\def \deftf#1{\ensuremath{{\cal F}[#1]}}
%\def \deftf#1{\ensuremath{{\rm FT}[#1]}}
\def \tf#1{\ensuremath{\widetilde{#1}}}
\def \tf#1{\ensuremath{\underline{#1}}}
\def \itf#1{\ensuremath{{\cal F}^{-1}#1}}
\def \xl{\ensuremath{x_\lambda}} % spatial frequency
\def \yl{\ensuremath{y_\lambda}} % spatial frequency
\def \ul{\ensuremath{u_\lambda}} % spatial frequency
\def \thl{\ensuremath{\theta_\lambda}} % reciprocal coordinate
%
% Quantum mechanics
%
\def \vect#1{\ensuremath{\vec{#1}}}
\def \op#1{\ensuremath{\hat{#1}}}
\def \ham{\ensuremath{{\cal H}}}
\def \wftot{\ensuremath{\Psi}}
\def \wfsp{\ensuremath{\phi}}
\def \wfspin{\ensuremath{\sigma}}
\def \wf{\ensuremath{\psi}}
\def \rmas{\ensuremath{\widetilde{m}}} % Reduced mass
\def \elec{\ensuremath{\rm e^-}}
%
% Angular momenta
%
\def \am{\ensuremath{\textsf{AM}}}
\def \oam{\ensuremath{\ell}}
\def \voam{\ensuremath{\vect{\ell}}}
\def \vl{\vect{l}}
\def \vs{\vect{s}}
\def \vj{\vect{j}}
\def \vi{\vect{i}}
\def \vf{\vect{f}}
\def \vli{\ensuremath{\vect{l}_i}}
\def \vsi{\ensuremath{\vect{s}_i}}
\def \vji{\ensuremath{\vect{j}_i}}
\def \vL{\vect{L}}
\def \vS{\vect{S}}
\def \vJ{\vect{J}}
\def \vI{\vect{I}}
\def \vF{\vect{F}}
\def \vr{\ensuremath{{\vect{r}}}}
\def \vR{\ensuremath{{\vect{R}}}}
%
\def \vbint{\ensuremath{\vec{B}_{\rm int}}}
\def \epot{\ensuremath{{\cal E}}}
\def \vso{\ensuremath{V_{\rm s-o}}}
%----------------------------------
%
% Radiation and photometry
%
% Units
\def \jy{\ensuremath{{\rm Jy}}}
\def \jysr{\ensuremath{{{\,\rm Jy\,sr^{-1}}}}}
\def \Mjysr{\ensuremath{{{\,\rm MJy\,sr^{-1}}}}}
\def \mjybeam{\ensuremath{{{\,\rm mJy/beam}}}}
\def \jkms{\ensuremath{{\,\jy\,\kms}}}
\def \lumsi{\ensuremath{{\,\rm W\,\mm}}}
\def \lumcgs{\ensuremath{{\,\rm erg\,\cc}}}
\def \fluxsi{\ensuremath{{\,\rm W\,\mm}}}
\def \intintsi{\ensuremath{{\,\rm W\,\mm\,sr^{-1}}}}
\def \intintcgs{\ensuremath{{\,\rm erg\pers\,\cm\,sr^{-1}}}}
\def \fluxcgs{\ensuremath{{\,\rm erg\,s^{-1}\,cm^{-2}}}}
\def \fdenscgs{\ensuremath{{\,\rm erg\,s^{-1}\,cm^{-2}\,Hz^{-1}}}}
\def \fdenssi{\ensuremath{{\,\rm W\,m^{-2}\,Hz^{-1}}}}
\def \ispecsi{\ensuremath{{\,\rm W\,m^{-2}\,Hz^{-1}\,sr^{-1}}}}
\def \ispecsiwl{\ensuremath{{\,\rm W\,m^{-2}\,m^{-1}\,sr^{-1}}}}
\def \ispec{\ensuremath{{\,\rm erg\,s^{-1}\,cm^{-2}\,Hz^{-1}\,sr^{-1}}}}
\def \emiss{\ensuremath{{\,\rm erg\, s^{-1}\, cm^{-3}}}}
\def \emisscoef{\ensuremath{{\,\rm erg\, s^{-1}\, cm^{-3}\,sr^{-1}\,Hz^{-1}}}}
\def \ergccc{\ensuremath{{\,\rm erg\, cm^{-3}}}}
\def \ergs{\ensuremath{{\,\rm erg\, s}}}
\def \jous{\ensuremath{{\,\rm J\, s}}}
%
\def \aul{\ensuremath{A_{ul}}}
\def \bul{\ensuremath{B_{ul}}}
\def \blu{\ensuremath{B_{lu}}}
\def \cul{\ensuremath{C_{ul}}}
\def \clu{\ensuremath{C_{lu}}}
\def \gul{\ensuremath{{\gamma_{ul}}}}
\def \glu{\ensuremath{{\gamma_{lu}}}}
\def \inu{\ensuremath{I_\nu}}
\def \ibg{\ensuremath{I_{\rm bg}}}
\def \jnu{\ensuremath{J_\nu}}
\def \anu{\ensuremath{{\alpha_\nu}}}
\def \knu{\ensuremath{{\kappa_\nu}}}
\def \snu{\ensuremath{{S_\nu}}}
\def \fnu{\ensuremath{{F_\nu}}}
\def \bnu{\ensuremath{B_\nu}}
\def \pnu{\ensuremath{p_\nu}}
\def \Pnu{\ensuremath{P_\nu}}
\def \efft{\ensuremath{\widetilde{T}}}
\def \etbr{\ensuremath{\widetilde{T}_{\rm B}}}
\def \etbg{\ensuremath{\widetilde{T}_{\rm bg}}}
\def \etex{\ensuremath{\widetilde{T}_{\rm ex}}}
\def \etkin{\ensuremath{\widetilde{T}_{\rm kin}}}
\def \nc{\ensuremath{n_{\rm crit}}}
\def \d{{\ud}}
\def \sr{\ensuremath{{\rm sr^{-1}}}}
\def \jbar{\ensuremath{\overline{J}}}
\def \udot#1{\ensuremath{\dot{#1}}}
\def \mbol{\ensuremath{m_{\rm bol}}}
\def \Mbol{\ensuremath{M_{\rm bol}}}
\def \lbol{\ensuremath{L_{\rm bol}}}
\def \teff{\ensuremath{T_{\rm eff}}}
%-----------------------------------------------
%
% Radio astronomy
%
%
\newcommand \tante{\ensuremath{T_{\rm A}}}
\newcommand \tant{\ensuremath{T_{{\rm A}}^\star}}
\newcommand \tmb{\ensuremath{{T_{{\rm mb}}}}}
\newcommand \tmbc{\ensuremath{T_{{\rm mb,c}}}}
\newcommand \feff{\ensuremath{F_{{\rm{eff}}}}}
\newcommand \beff{\ensuremath{B_{{\rm{eff}}}}}

\def \off{{\tt OFF}}
\def \terr{\ensuremath{T_{\rm err}}}
\def \tA{\ensuremath{T_{\rm A}}}
\def \tB{\ensuremath{T_{\rm B}}}
\def \tR{\ensuremath{T_{\rm R}}}
\def \tantc{\ensuremath{T_{\rm A,c}^*}}
\def \tmbc{\ensuremath{T_{\rm mb,c}}}
\def \mb{\ensuremath{{\om_{\rm mb}}}}
\def \sou{\ensuremath{{\om_{\rm S}}}}
\def \tbr{\ensuremath{T_{{\rm B}}}}
\def \tkin{\ensuremath{T_{{\rm kin}}}}
\def \texc{\ensuremath{T_{{\rm ex}}}}
\def \tgas{\ensuremath{T_{{\rm gas}}}}
\def \tdust{\ensuremath{T_{\rm dust}}}
\def \tbg{\ensuremath{T_{{\rm bg}}}}
\def \aper{\ensuremath{{\cal A}}}  % Complexe aperture function
\def \ffield{\ensuremath{f}}       % Far-field pattern
\def \pp{\ensuremath{{\cal P}}}    % Far-field power pattern
\def \ppnu{\ensuremath{{\cal P}_\nu}}    % Far-field power pattern
\def \otf{\ensuremath{{\cal T}}}   % Telescope transfer function
\def \eant{\ensuremath{E_{\rm aper}}}
\def \efar{\ensuremath{E_{\rm ff}}}
\def \pbeam{\ensuremath{{\cal P}(\Omega)}}
\def \pmb{\ensuremath{{\cal P}_0(\Omega)}}
\def \perr{\ensuremath{{\cal P}_e(\Omega)}}
\def \perrk{\ensuremath{{\cal P}_{e,k}(\Omega)}}
\def \pwall{\ensuremath{{\cal P}_{4\pi}}}
\def \pwhalf{\ensuremath{{\cal P}_{2\pi}}}
\def \pwmb{\ensuremath{{\cal P}_{\rm mb}}}
\def \pwsou{\ensuremath{{\cal P}_S}}
\def \tsou{\ensuremath{T_{\rm sou}}}
\def \tgr{\ensuremath{T_{\rm gr}}}
\def \tcal{\ensuremath{T_{{\rm cal}}}}
\def \tsys{\ensuremath{T_{\rm sys}}}
\def \tsky{\ensuremath{T_{\rm sky}}}
\def \trec{\ensuremath{T_{\rm rec}}}
\def \temi{\ensuremath{T_{\rm sky}}}
\def \tspil{\ensuremath{T_{\rm spillover}}}
\def \tatm{\ensuremath{T_{\rm atm}}}
\def \thot{\ensuremath{T_{\rm hot}}}
\def \tcol{\ensuremath{T_{\rm col}}}
\def \etau{\ensuremath{e^{-\tau_\nu}}}
\def \csou{\ensuremath{C_{\rm sou}}}
\def \catm{\ensuremath{C_{\rm atm}}}
\def \chot{\ensuremath{C_{\rm hot}}}
\def \ccol{\ensuremath{C_{\rm col}}}
\def \nulo{\ensuremath{\nu_{\rm LO}}}
\def \nusky{\ensuremath{\nu_{\rm sky}}}
\def \nuif{\ensuremath{\nu_{\rm IF}}}
\def \philo{\ensuremath{\Phi_{\rm LO}}}
\def \phisky{\ensuremath{\Phi_{\rm sky}}}
%
% Interferometry
\def \vis{\ensuremath{{\cal V}}}
%
%
%----------------------------------
% Editing
\def \xe{\ensuremath{x_e}}
\def \Left{\textit{Left}}
\def \Right{\textit{Right}}
\def \mc#1#2{\multicolumn{#1}{c}{#2}}
\def \hlign#1#2{\noindent\centerline{\rule{#1\textwidth}{#2pt}\goodbreak}}
\def \fullw{1.0\hsize}
\def \fullh{0.85\textheight}
\def \fulh{0.75\textheight}
\def \mcite#1{{\centerline{\tiny\cite{#1}}}}
%\def \subtitle#1{\par{\centerline{\tiny #1}}}
\def \note#1{{\scriptsize #1}}
\def \fnote#1{{\par\noindent\tiny #1}}
\def \Htitle#1{\centerline{\Large \textbf{#1}}\hlign{1}{2}\bigskip}
\newcommand\entry[1]{\noindent\textbf{#1}}
%\newcommand\htitle#1{%
%  \centerline{\Large \textbf{#1}}\hlign{1}{1}\tableofcontents\hlign{1}{1}}

\newcommand\htitle[1]{%
  \begin{center}
    \begin{minipage}[c]{0.8\hsize}
      \centering
      \Large
      \textbf{#1}
    \end{minipage}
  \end{center}\hlign{1}{1}\tableofcontents\hlign{1}{1}}

\newcommand \idx[1]{#1\index{#1}}
\newcommand \iidx[2]{#2\index{#1!#2}}
\newcommand \iiidx[2]{#1 #2\index{#1!#2}}
%\newcommand \refeq[1]{Eq.~(\ref{eq:[1]})}
\newcommand \req[1]{Equ.~(\ref{eq:#1})}
\newcommand \reqs[2]{Eqs.~(\ref{eq:#1})--(\ref{eq:#2})}
\newcommand \rsec[1]{Sect.~\ref{sec:#1}}
\newcommand \rtab[1]{Table~\ref{tab:#1}}
\newcommand \rfig[1]{Fig.~\ref{fig:#1}}


==> journal_short.tex <==
\def \aal{A\&A Letters}
\def \aap{A\&A}
\def \aaps{A\&AS}
\def \aapr{Astron. Astrophys. Rev.}
\def \apss{Astroph. \& Sp. Sc.}
\def \aj{AJ}
\def \apj{ApJ}
\def \apjl{ApJL}
\def \apjs{ApJS}
\def \apl{Astrop. Lett.}
\def \araa{ARA\&A}
\def \bain{Bull. Astr. Inst. Netherlands}
\def \chemrev{Chemical Reviews}
\def \gca{Geochim. Cosmochim. Ac.}
\def \icarus{Icarus}
\def \inprep{\textit{in prep.}}
\def \jfm{JFM}
\def \mnras{MNRAS}
\def \nat{Nature}
\def \pasj{PASJ}
\def \pasp{PASP}
\def \pccp{Phys. Chem. Chem. Phys.}
\def \ppvi{Protostars \& Planets VI}
\def \prl{PRL}
\def \pra{Phys Rev A}
\def \prb{Phys Rev B}
\def \prc{Phys Rev C}
\def \prd{Phys Rev D}
\def \qjras{Q. Jl R. astr. Soc.}
\def \rmp{Rev. Mod. Phy.}
\def \phypla{Phys. Plasmas}
\def \phyflu{Phys. Fluids}
\def \jphysb{Jour. of Physics B}
\def \pieee{Proc. IEEE}
\def \fcp{Fundamental Cosmic Physics}
\def \actaa{Acta Astronomica}
\def \ssr{Space Sci Rev}
\def \sci{Science}
\def \sub{submitted}
\def \epsl{E\&PS Letters}
\def \euphysb{Eur. Phys. J. B.}
\def \jcp{JCP}
\def \jpca{JPCA}
\def \mps{Meteor. \& Plan. Sc.}
\def \pnas{PNAS}
\def \jms{Jour. Molec. Spec.}
\def \pccp{PCCP}
\def \arfm{AR Flu Mech}
\def \molphys{Mol. Phys.}


==> latexfigs.tex <==
% Lenghts

\def\fullw{0.95\hsize}
\def\fullh{0.85\textheight}
\def\fulh{0.7\textheight}
% 
% Environments for figures
%
\def\land#1#2{\includegraphics[width=#1\hsize]{#2}}
\newcommand\port[2]{{\includegraphics[height=#1\textheight]{#2}}}
\newcommand\onefig[2]{\includegraphics[#1]{#2}}
\newcommand\hfig[2]{\includegraphics[width=#1\textwidth]{{#2}}}
\newcommand\vfig[2]{\includegraphics[height=#1\textheight]{{#2}}}
\newcommand\rotfig[3]{\includegraphics[angle=#1,width=#2\textheight]{#3}}
\newcommand\onehfig{\hfig}
\newcommand\onevfig{\vfig}

